Fast-moving object counting with an event camera

This paper proposes the use of an event camera as a component of a vision system that enables counting of fast-moving objects - in this case, falling corn grains. These type of cameras transmit information about the change in brightness of individual pixels and are characterised by low latency, no motion blur, correct operation in different lighting conditions, as well as very low power consumption. The proposed counting algorithm processes events in real time. The operation of the solution was demonstrated on a stand consisting of a chute with a vibrating feeder, which allowed the number of grains falling to be adjusted. The objective of the control system with a PID controller was to maintain a constant average number of falling objects. The proposed solution was subjected to a series of tests to determine the correctness of the developed method operation. On their basis, the validity of using an event camera to count small, fast-moving objects and the associated wide range of potential industrial applications can be confirmed.

==> sn-bibliography.tex <==
\begin{thebibliography}{50}

% \bibitem{lee2017real} Shih-Hsiung Lee, Chu-Sing Yang, A real time object recognition and counting system for smart industrial camera sensor, IEEE Sensors Journal, vol. 17 (2017), 2516--2523


\bibitem{gallego2022}Gallego, G., Delbrück, T., Orchard, G., Bartolozzi, C., Taba, B., Censi, A., Leutenegger, S., Davison, A., Conradt, J., Daniilidis, K. \& Scaramuzza, D. Event-Based Vision: A Survey. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. \textbf{44}, 154-180 (2022).

\bibitem{LiPoDe}Lichtsteiner, P., Posch, C. \& T., D. A 128× 128 120 dB 15 us Latency Asynchronous Temporal Contrast Vision Sensor. {\em IEEE Journal Of Solid-State Circuits 43(2):566 - 576}. (2008).

\bibitem{kim2016}Kim, H., Leutenegger, S. \& Davison, A. Real-Time 3D Reconstruction and 6-DoF Tracking with an Event Camera. {\em Computer Vision – ECCV 2016}. pp. 349-364 (2016).

\bibitem{padala2018}Padala, V., Basu, A. \& Orchard, G. A Noise Filtering Algorithm for Event-Based Asynchronous Change Detection Image Sensors on TrueNorth and Its Implementation on TrueNorth. {\em Frontiers In Neuroscience}. \textbf{12} (2018).

\bibitem{lee2017real}Lee, S. \& Yang, C. A real time object recognition and counting system for smart industrial camera sensor. {\em IEEE Sensors Journal}. \textbf{17}, 2516-2523 (2017).

\bibitem{baygin2018image}Baygin, M., Karakose, M., Sarimaden, A. \& Akin, E. An image processing based object counting approach for machine vision application. {\em ArXiv Preprint ArXiv:1802.05911}. (2018).

\bibitem{liu2017fast}Liu, J. \& Na, W. Fast moving object counting from video. {\em 2017 International Symposium On Intelligent Signal Processing And Communication Systems (ISPACS)}. pp. 337-340 (2017).

\bibitem{lee2012}Lee, K., Tsai, L. \& Hung, P. Fast People Counting Using Sampled Motion Statistics. {\em 2012 Eighth International Conference On Intelligent Information Hiding And Multimedia Signal Processing}. pp. 162-165 (2012).

\bibitem{saidon2021automatic}Saidon, M., Mustafa, W., Rajasalavam, V. \& Khairunizam, W. Automatic People Counting System Using Aerial Image Captured by Drone for Event Management. {\em Intelligent Manufacturing And Mechatronics}. pp. 51-65 (2021).

\bibitem{liu2021}Liu, C., Huynh, D., Sun, Y., Reynolds, M. \& Atkinson, S. A Vision-Based Pipeline for Vehicle Counting, Speed Estimation, and Classification. {\em IEEE Transactions On Intelligent Transportation Systems}. \textbf{22}, 7547-7560 (2021).

\bibitem{wu2021}Wu, H., Wang, Y., Ma, H., Li, B. \& Jin, Y. Vision Based Real-time High-accuracy Automatic Counting with Applications for Smart Pharmacy. {\em 2021 40th Chinese Control Conference (CCC)}. pp. 6429-6435 (2021).

\bibitem{belbachir2010real}Belbachir, A., Schraml, S. \& Brändle, N. Real-time classification of pedestrians and cyclists for intelligent counting of non-motorized traffic. {\em 2010 IEEE Computer Society Conference On Computer Vision And Pattern Recognition-Workshops}. pp. 45-50 (2010).



% \bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

% \bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

% \bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

% \bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

% \bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

% \bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

% \bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


